Performance Conditioning for Diffusion-Based Multi-Instrument Music Synthesis

Generating multi-instrument music from symbolic music representations is an important task in Music Information Retrieval (MIR). A central but still largely unsolved problem in this context is musically and acoustically informed control in the generation process. As the main contribution of this work, we propose enhancing control of multi-instrument synthesis by conditioning a generative model on a specific performance and recording environment, thus allowing for better guidance of timbre and style. Building on state-of-the-art diffusion-based music generative models, we introduce performance conditioning - a simple tool indicating the generative model to synthesize music with style and timbre of specific instruments taken from specific performances. Our prototype is evaluated using uncurated performances with diverse instrumentation and achieves state-of-the-art FAD realism scores while allowing novel timbre and style control. Our project page, including samples and demonstrations, is available at benadar293.github.io/midipm

==> tables/table_all_metrics.tex <==
\begin{table*}[t!]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
% & \multicolumn{4}{|c|}{FAD VGGish} & \multicolumn{4}{|c|}{FAD TRILL} & \multicolumn{2}{|c|}{\multirow{2}{*}{ID Acc.\% (TRILL)}} & \multicolumn{2}{|c|}{Transcription} \\
& \multicolumn{4}{|c|}{FAD VGGish} & \multicolumn{4}{|c|}{FAD TRILL} & \multicolumn{2}{|c|}{ID Acc.\% (TRILL)} & \multicolumn{2}{|c|}{Transcription} \\
\cline{1-9}
Model & \multicolumn{2}{|c|}{Group} & \multicolumn{2}{|c|}{All} & \multicolumn{2}{|c|}{Group} & \multicolumn{2}{|c|}{All} & \multicolumn{2}{|c|}{Top-1/Top-3} & \multicolumn{2}{|c|}{Note / Note+Inst.} \\
\hline
& Con. & Unc. & Con. & Unc. & Con. & Unc. & Con. & Unc. & Con. & Unc. & Con. & Unc. \\
\hline
T5A & 5.29 & 7.7 & 3.09 & 4.2 & 0.33 & 0.54 & 0.09 & 0.15 & 57.4/80.0 & 9.7/21.3 & 65.3/50.3 & 58.5/34.2\\
\hline
T5B & 5.46 & 5.83 & 3.53 & 3.98 & 0.35 & 0.43 & 0.09 & 0.12 & 67.7/89.7 & 35.5/60.0 & 63.2/47.1& 59.1/36.0 \\
\hline
% 5.12 & & 3.94 & & 0.33 & & 0.11
% 7.06 & & 3.37 & & 0.5 & & 0.12
UNet & 5.12 & 7.06 & 3.94 & 3.37 & 0.33 & 0.5 & 0.11 & 0.12 & 56.1/72.9 & 13.5/29.7 & 60.8/45.3 & 62.8/46.3 \\
\hline
% UNetL & 5.2 & 6.78 & 3.93 & 3.78 & 0.33 & 0.49 & 0.1 & 0.13 & 51.0/70.3 & 14.2/29.0 & 60.2/45.2 & 62.4/46.6 \\
% \hline

%% with VGGish classification:
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% & \multicolumn{6}{|c|}{VGGish} & \multicolumn{6}{|c|}{TRILL} & \multicolumn{2}{|c|}{Transcription} \\
% \hline
% & \multicolumn{6}{|c|}{VGGish} & \multicolumn{6}{|c|}{TRILL} & \multicolumn{2}{|c|}{Transcription} \\
% \hline
% Model & \multicolumn{2}{|c|}{FAD (Group)} & \multicolumn{2}{|c|}{FAD (All)} & \multicolumn{2}{|c|}{ID Acc.\%} & \multicolumn{2}{|c|}{FAD (Group)} & \multicolumn{2}{|c|}{FAD (All)} & \multicolumn{2}{|c|}{ID Acc.\%} & \multicolumn{2}{|c|}{N / N\&I / F} \\
% \hline
% & Con. & Unc. & Con. & Unc. & Con. & Unc. & Con. & Unc. & Con. & Unc. & Con. & Unc. & Con. & Unc. \\
% \hline
% T5A & 5.29 & 7.7 & 3.09 & 4.2 & & & 0.33 & 0.54 & 0.09 & 0.15 & 99 & 100\% \\
% \hline
% T5B & 5.46 & 5.83 & 3.53 & 3.98 & 34.9/61.3 & 28.4/47.1 & 0.35 & 0.43 & 0.09 & 0.12 & 67.7/89.7 & 35.5/60.0 & & 100\% \\
% \hline
% U-Net & Synth & \xmark & 99 & 0\% \\
% \hline
% U-Net L & Piano & \xmark & 99 & 100\% \\
% \hline
\end{tabular}
\end{center}
\caption{Results for all models. T5A is the 'Base' model from~\cite{DBLP:journals/corr/abs-2206-05408}, with adding ID embeddings to the decoder. T5B also has ID embeddings in the note encoder. We fix the note condition strength (guidance weight) to 1.25, and for each metric compare ID condition of strength 1.25 ('Con.') to ID strength 0 ('Unc.'). It can be seen that ID conditioning drastically improves FAD, both groupwise, including ID classification, and over the entire set, and also transcription accuracy. ID embeddings in the T5 encoder (T5B) improve most metrics.}
\label{table:all_metrics}
\end{table*}

==> tables/table_all_metrics_one_column.tex <==
\begin{table}[t!]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
% & \multicolumn{4}{|c|}{FAD VGGish} & \multicolumn{4}{|c|}{FAD TRILL} & \multicolumn{2}{|c|}{\multirow{2}{*}{ID Acc.\% (TRILL)}} & \multicolumn{2}{|c|}{Transcription} \\
& \multicolumn{2}{|c|}{VGGish$\downarrow$} & \multicolumn{2}{|c|}{TRILL$\downarrow$} & Acc.\%& Transc.\\
\cline{2-5}
 & Grp & All & Grp & All & Top-1/3$\uparrow$ & N/N+I$\uparrow$ \\
\hline
\multicolumn{7}{|c|}{with Performance-Conditioning}\\
\hline
TA & \underline{5.29} & \textbf{3.09} & \textbf{\underline{0.33}} & \textbf{\underline{0.09}} & \underline{57.4}/\underline{80.0} & \textbf{65.3}/\textbf{50.3} \\
% \hline
TB & 5.46 & \underline{3.53} & 0.35 & \textbf{\underline{0.09}} & \textbf{67.7}/\textbf{89.7} & \underline{63.2}/\underline{47.1} \\
% \hline
U & \textbf{5.12} & 3.94 & \textbf{\underline{0.33}} & 0.11 & 56.1/72.9 & 60.8/45.3 \\
\hline
\multicolumn{7}{|c|}{w/o Performance-Conditioning}\\
\hline
TA & 7.7 & 4.2 & 0.54 & 0.15 & 9.7/21.3 & 58.5/34.2 \\
% \hline
TB & 5.83 & 3.98 & 0.43 & 0.12 & 35.5/60.0 & 59.1/36.0 \\
% \hline
U & 7.06 & 3.37 & 0.5 & 0.12 & 13.5/29.7 & 62.8/46.3 \\
\hline
\end{tabular}
\end{center}
\caption{Results for all metrics -- FAD (VGGish, TRILL), performance classification accuracy with TRILL FAD-nearest (Acc.\%), and transcription accuracy - note (N) and note-with-instrument (N+I). TA, TB, and U are the T5A, T5B, and U-Net models, respectively.
% TA (T5A) is the 'Base' model from~\cite{DBLP:conf/ismir/HawthorneSRZGME22}, with performance embeddings added to the decoder. TB (T5B) also has performance embeddings in the note encoder. 
We use note condition strength (CFG weight) of 1.25, and compare performance condition of strength 1.25 (upper rows) to no performance condition (lower rows). It can be seen that the performance conditioning has a dramatic effect on classification and group FAD (Grp), implying that performance-specific characteristics are achieved. Note that the TA, TB models without performance conditioning are equivalent to the model of~\cite{DBLP:conf/ismir/HawthorneSRZGME22}.}
\label{table:all_metrics}
\end{table}

==> tables/table_metrics_fad_group_AB.tex <==
\begin{table}[t!]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
& \multicolumn{4}{|c|}{FAD(Group)$\downarrow$} & \multicolumn{2}{|c|}{Perf. Acc.\%} \\
\cline{2-5}
 & \multicolumn{2}{|c|}{VGGish} & \multicolumn{2}{|c|}{TRILL} & \multicolumn{2}{|c|}{Top-1/3$\uparrow$} \\
\hline
P Con. & w/ & w/o & w/ & w/o & w/ & w/o \\
% \hline
% T5A & \underline{5.3} & 7.7 & \textbf{\underline{0.33}} & 0.54 & \underline{57.4}/\underline{80.0} & 9.7/21.3 \\
% % \hline
% T5B & 5.5 & 5.8 & 0.35 & 0.43 & \textbf{67.7}/\textbf{89.7} & 35.5/60.0 \\
% % \hline
% U-Net & \textbf{5.1} & 7.1 & \textbf{\underline{0.33}} & 0.5 & 56.1/72.9 & 13.5/29.7 \\
% \hline
\hline
T5A & \underline{5.3} & 7.7 & \textbf{\underline{0.33}} & 0.54 & \underline{57}/\underline{80}\% & 10/21\% \\
% \hline
T5B & 5.5 & 5.8 & 0.35 & 0.43 & \textbf{68}/\textbf{90}\% & 36/60\% \\
% \hline
U-Net & \textbf{5.1} & 7.1 & \textbf{\underline{0.33}} & 0.5 & 56/73\% & 14/30\% \\
\hline

% Perf. & \multirow{2}{*}{w/} & \multirow{2}{*}{w/o} & \multirow{2}{*}{w/} & \multirow{2}{*}{w/o} & \multirow{2}{*}{w/} & \multirow{2}{*}{w/o} \\
% Cond. &&&&&& \\

% \multicolumn{4}{|c|}{with Performance-Conditioning}\\
% % \hline
% T5B & 5.46 & 5.83 & 0.35 & 0.43 & \textbf{67.7}/\textbf{89.7} & 35.5/60.0 \\
% % \hline
% U-Net & \textbf{5.12} & 7.06 & \textbf{\underline{0.33}} & 0.5 & 56.1/72.9 & 13.5/29.7 \\
% \hline
% \multicolumn{4}{|c|}{w/o Performance-Conditioning}\\
% \hline


% T5A & \underline{5.29} & 7.7 & \textbf{\underline{0.33}} & 0.54 & \underline{57.4}/\underline{80.0} & 9.7/21.3 \\
% % \hline
% T5B & 5.46 & 5.83 & 0.35 & 0.43 & \textbf{67.7}/\textbf{89.7} & 35.5/60.0 \\
% % \hline
% U-Net & \textbf{5.12} & 7.06 & \textbf{\underline{0.33}} & 0.5 & 56.1/72.9 & 13.5/29.7 \\
% \hline
% \multicolumn{4}{|c|}{w/o Performance-Conditioning}\\
% \hline
% T5A & 7.7 & 0.54 & 9.7/21.3 \\
% % \hline
% T5B & 5.83 & 0.43 & 35.5/60.0 \\
% % \hline
% U-Net & 7.06 & 0.5 & 13.5/29.7 \\
% \hline
\end{tabular}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \multirow{2}{*}{Model} & \multicolumn{2}{|c|}{FAD(Grp)$\downarrow$} & Acc.\% \\
% \cline{2-4}
%  & VG & TR & Top-1/3$\uparrow$ \\
% \hline
% \multicolumn{4}{|c|}{with Performance-Conditioning}\\
% \hline
% T5A & \underline{5.29} & \textbf{\underline{0.33}} & \underline{57.4}/\underline{80.0} \\
% % \hline
% T5B & 5.46 & 0.35 & \textbf{67.7}/\textbf{89.7} \\
% % \hline
% U-Net & \textbf{5.12} & \textbf{\underline{0.33}} & 56.1/72.9 \\
% \hline
% \multicolumn{4}{|c|}{w/o Performance-Conditioning}\\
% \hline
% T5A & 7.7 & 0.54 & 9.7/21.3 \\
% % \hline
% T5B & 5.83 & 0.43 & 35.5/60.0 \\
% % \hline
% U-Net & 7.06 & 0.5 & 13.5/29.7 \\
% \hline
% \end{tabular}
\end{center}
% \vspace{-.4cm}
\caption{Results for Group-FAD, and performance classification accuracy with TRILL FAD-nearest (Perf. Acc.\%). 
% We use note condition strength (CFG weight) of 1.25, and compare performance condition of strength 1.25 (upper rows) to no performance condition (lower rows). 
% {\color{red}leave this sentence out: Performance conditioning (P Con.) has a dramatic effect on performance classification accuracy and group-FAD, implying that performance-specific characteristics are achieved.}
The best result in each metric is bold, and the next-best is underlined.
% Note that the T5A, T5B models without performance conditioning are equivalent to the model of~\cite{DBLP:conf/ismir/HawthorneSRZGME22}.
}
% \vspace{-.4cm}
\label{table:fad_group}
\end{table}

==> tables/table_metrics_fad_transcription_AB.tex <==
\begin{table}[t!]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Model} & \multicolumn{4}{|c|}{FAD(All)$\downarrow$} & \multicolumn{2}{|c|}{Transcription}\\
\cline{2-5}
& \multicolumn{2}{|c|}{VGGish} & \multicolumn{2}{|c|}{TRILL} & \multicolumn{2}{|c|}{N/N+I$\uparrow$} \\
\hline
P Con. & w/ & w/o & w/ & w/o & w/ & w/o \\
\hline
T5A & \textbf{3.1} & 4.0 & \textbf{\underline{0.09}} & 0.15 & \textbf{65}/\textbf{50}\% & 61/36\% \\
T5B & \underline{3.5} & 3.9 & \textbf{\underline{0.09}} & 0.12 & \underline{63}/\underline{47}\% & 62/38\% \\
U-Net & 3.9 & 3.4 & 0.11 & 0.12 & 62/46\% & 63/47\% \\
\hline
% \hline
% P Cond. & w/ & w/o & w/ & w/o & w/ & w/o \\
% \hline
% T5A & \textbf{3.1} & 4.0 & \textbf{\underline{0.09}} & 0.15 & \textbf{65}/\textbf{50}/\underline{66} & 61/36/\textbf{67} \\
% T5B & \underline{3.5} & 3.9 & \textbf{\underline{0.09}} & 0.12 & \underline{63}/\underline{47}/62 & 62/38/65 \\
% U-Net & 3.9 & 3.4 & 0.11 & 0.12 & 62/46/64 & 63/47/65 \\
% \hline
% & \multicolumn{5}{|c|}{w/o Performance-Conditioning}\\
% \hline
% % T5A & 4.2 & 0.15 & 58.5 & 34.2 & 66.1 \\
% % midi cfg 1.5 id cfg 0:
% T5A & 4.0 & 0.15 & 61/36/\textbf{67} \\
% % \hline
% % T5B & 3.98 & 0.12 & 59.1 & 36.0 \\
% % midi cfg 1.5 id cfg 0:
% T5B & 3.89 & 0.12 & 62/38/65 \\
% % \hline
% % U-Net & 3.37 & 0.12 & 62.8 & 46.3 \\
% U-Net & 3.37 & 0.12 & 63/47/65 \\
% \hline
% \hline
% \multirow{2}{*}{Model} & \multicolumn{2}{|c|}{FAD(All)$\downarrow$} & \multicolumn{3}{|c|}{Transcription}\\
% \cline{2-6}
% & VG & TR & N & N+I & Fr \\
% \cline{2-5}
% \hline
% & \multicolumn{5}{|c|}{with Performance-Conditioning}\\
% \hline
% \multirow{2}{*}{Model} & \multicolumn{2}{|c|}{FAD(All)$\downarrow$} & \multicolumn{3}{|c|}{Transcription}\\
% \cline{2-6}
% & VG & TR & N/N+I/Fr \\
% \cline{2-5}
% \hline
% & \multicolumn{5}{|c|}{with Performance-Conditioning}\\
% \hline
% T5A & \textbf{3.09} & \textbf{\underline{0.09}} & \textbf{65.3} & \textbf{50.3} & \underline{65.8} \\
% % \hline
% T5B & \underline{3.53} & \textbf{\underline{0.09}} & \underline{63.2} & \underline{47.1} & 62.0 \\
% % \hline
% % U-Net & 3.94 & 0.11 & 60.8 & 45.3 \\
% % midi cfg 1.5 id cfg 1.5:
% U-Net & 3.94 & 0.11 & 61.8 & 46.2 & 64.1 \\
% \hline
% & \multicolumn{5}{|c|}{w/o Performance-Conditioning}\\
% \hline
% % T5A & 4.2 & 0.15 & 58.5 & 34.2 & 66.1 \\
% % midi cfg 1.5 id cfg 0:
% T5A & 4.0 & 0.15 & 61.2 & 36.2 & \textbf{67.2} \\
% % \hline
% % T5B & 3.98 & 0.12 & 59.1 & 36.0 \\
% % midi cfg 1.5 id cfg 0:
% T5B & 3.89 & 0.12 & 62.0 & 38.4 & 65.0 \\
% % \hline
% % U-Net & 3.37 & 0.12 & 62.8 & 46.3 \\
% U-Net & 3.37 & 0.12 & 63.1 & 46.6 & 65.4 \\
% \hline


% & \multicolumn{4}{|c|}{FAD VGGish} & \multicolumn{4}{|c|}{FAD TRILL} & \multicolumn{2}{|c|}{\multirow{2}{*}{ID Acc.\% (TRILL)}} & \multicolumn{2}{|c|}{Transcription} \\
% & \multicolumn{2}{|c|}{VGGish$\downarrow$} & \multicolumn{2}{|c|}{TRILL$\downarrow$} & Acc.\%& Transc.\\
% \cline{2-5}
%  & Grp & All & Grp & All & Top-1/3$\uparrow$ & N/N+I$\uparrow$ \\
\end{tabular}
\end{center}
% \vspace{-.4cm}
\caption{Results for All-FAD, and transcription accuracy for note (N) and note-with-instrument (N+I). For each metric, the best result is bold, and the next-best is underlined.
% We use note condition strength (CFG weight) of 1.25, and compare performance condition of strength 1.25 (upper rows) to no performance condition (lower rows). 
% {\color{red}end caption here and leave the rest out} 
% While performance conditioning (P Con.) has a positive effect on these metrics, the most dramatic effect is in performance classification and group FAD (Table~\ref{table:fad_group}).
}
% \vspace{-.4cm}
\label{table:fad_transcription}
\end{table}
